Analysis of linear Boussinesq-type models coupled with static interfaces

We derive a new approach to analyze the coupling of linear Boussinesq and Saint-Venant shallow water wave equations in the case where the interface remains at a constant position in space. We propose a one-way coupling model as a reference, which allows us to obtain an analytical solution, prove the well-posedness of the original coupled model and compute what we call the coupling error-a quantity that depends solely on the choice of transmission conditions at the interface. We prove that this coupling error is asymptotically small for a certain class of data and discuss its role as a proxy for the full error with respect to the 3D water wave problem. Additionally, we highlight that this error can be easily computed in other scenarios. We show that the coupling error consists of reflected waves and argue that this explains some previously unexplained spurious oscillations reported in the literature. Finally, we prove the well-posedness of the half-line linear Boussinesq problem.

==> analysishybrid.tex <==

\section{Space (vertical) interface}

\label{ch:hybrid}
Now we focus on the study of the linear hybrid model. To conduct the analysis, we begin by introducing the model and characterizing the coupling conditions that reformulate it as two coupled half-line problems \eqref{eq:half-line-problem}. Then, we proceed to derive formulas for its solution from where the Hadamard well-posedness and the coupling error--introduced in \textcolor{red}{Sec. x}--can be deduced. This derivation explains the (i) Small oscillations and (iii) Instabilities introduced in \textcolor{red}{sec. x}, while also proving the effect that the coupling conditions have on the approximation of the water wave problem, plus its relation to other features, such as absorbing boundary conditions, etc.



\subsection{Characterization of the coupling conditions}



The strategy for the analysis of the heterogeneous Cauchy problem \eqref{eq:hybrid-compact} is to reformulate it as two coupled homogeneous problems in the half-line:
\begin{equation}
    \left\{ \begin{array}{ll}
        \mathcal{L}_- \vect W_- = 0, &\quad \text{ in } Q_- \\ 
        \vect W_-(\cdot,0) = \vect W_0, &\quad \text{ in } \Omega_-
    \end{array}\right. \\ 
    \left\{ \begin{array}{ll}
        \mathcal{L}_+ \vect W_+ = 0, &\quad \text{ in } Q_+ \\ 
        \vect W_+(\cdot,0) = \vect W_0, &\quad \text{ in } \Omega_+
    \end{array}\right.
    \label{eq:hybrid-halflines}
\end{equation}
by finding coupling conditions such that the solution is preserved, \text{i.e.},  
\begin{equation}
    \begin{split}
        \vect W = \vect W_-, & \quad \text{ in } Q_- \\ 
        \vect W = \vect W_+, & \quad \text{ in } Q_+
    \end{split}
\end{equation}
with $\vect W$ solution to \eqref{eq:hybrid-compact} and $(\vect W_-, \vect W_+)$ solution of \eqref{eq:hybrid-halflines}. 
The next theorem reveals the coupling conditions that reformulate problem \eqref{eq:hybrid-compact} as an equivalent coupling of the two half-line problems \eqref{eq:hybrid-halflines}.

    
\begin{theorem}[Coupling conditions of the hybrid model]

    \label{th:hybrid-coupling-conditions}
    Suppose $\vect W=(\eta, u)$ is solution of \eqref{eq:hybrid-compact}, $\vect W_-=(\eta_-, u_-)$, $\vect W_+=(\eta_+, u_+)$ solve problems \eqref{eq:hybrid-halflines}, and the Laplace transforms of $u_-(,\cdot)$, $u_+(0,\cdot)$, $\partial_x u_-(0,\cdot)$, $\partial_x u_+(0,\cdot)$ exist. Then $\vect W_- = \vect W_{| \overline Q_-}$ and $\vect W_+ = \vect W_{| \overline{Q}_+}$ if and only if
\begin{equation}
    \begin{split}
        u_-(0,\cdot) = u_+(0,\cdot) \\ 
        \partial_x u_-(0,\cdot) = \partial_x u_+(0,\cdot)
    \end{split}
    \quad \text{ in }]0,T[
    \label{eq:coupling-conditions}
\end{equation}
\end{theorem}

\begin{proof}
     Let 
     $$\vect V_- = (\zeta_-,v_-) = \vect W_- - \vect W \quad \text{ in } \overline Q_-$$ 
     $$\vect V_+ = (\zeta_+,v_+) = \vect W_+ - \vect W \quad \text{ in} \overline Q_+$$ 
     then $\vect V_-$ and $\vect V_+$ satisfy \eqref{eq:hybrid-halflines} with 
     \begin{equation}
        \vect V_\pm(\cdot,0) = 0, \quad \text{ in }  \Omega_\pm
     \end{equation}
     
     ($\Rightarrow$): Assuming that $\vect W_- = \vect W_{| \overline Q_-}$ and $\vect W_+ = \vect W_{| \overline{Q}_+}$, then $v_-$ and $v_+$ are constant and equal to zero in $\overline{Q}_\pm$ as also are $\partial_x v_\pm$. Since both $\overline Q_\pm$ contain $\{x=0,t\in[0,T]\}$, we have that  $v_-(0,t)=v_+(0,t)=0$ and $\partial_x v_-(0,t)=\partial_x v_+(0,t)=0$. From the assumption that the Laplace transforms of $u_-(,\cdot), u_+(0,\cdot), \partial_x u_-(0,\cdot), \partial_x u_+(0,\cdot)$ exist, we deduce $\partial_x v_\pm(0,\cdot) = \partial_x u_\pm(0,\cdot) - \partial_x u(0,\cdot)=0$, hence \cref{eq:coupling-conditions} holds. 
   
    ($\Leftarrow)$:  On the other side, let us denote by $\hat{()}$ the Laplace transform. Let us also assume that the equations \eqref{eq:coupling-conditions} hold and let $\lambda_\pm(s)$ be such that 
    \begin{equation}
        \begin{split}
            v_-(x,s) &= \hat u_-(0,s) e^{\lambda_-(s)x},\quad (x,s) \in \Omega_- \times \mathbb{C}^+ \\
            v_+(x,s) &= \hat u_+(0,s)  e^{-\lambda_+(s)x},\quad (x,s) \in \Omega_+ \times \mathbb{C}^+ 
            \label{eq:half-hybrid-proof-solution}
        \end{split}
    \end{equation}
    as in \Cref{sec:laplace-halfline}. Because at $t=0$ $v_-$ and $v_+$ are null, from \eqref{eq:half-hybrid-proof-solution} we know that
    \begin{equation*}
        \begin{split}
            \partial_x \hat v_-(0,s) &= \lambda_-(s) \hat v_-(0,s)\\
            \partial_x \hat v_+(0,s) &= -\lambda_+(s) \hat v_+(0,s)                
        \end{split}
        \label{eq:abstract-transmission-conditions}
    \end{equation*}
    Substracting both equations in \eqref{eq:abstract-transmission-conditions} 
    \begin{equation*}
        \partial_x \hat v_-(0,s) - \partial_x \hat v_+(0,s) = (\lambda_-(s) \hat v_-(0,s) + \lambda_+(s) \hat v_+(0,s))
    \end{equation*}
    and, by definition of $v_\pm$, if the first equation of \eqref{eq:coupling-conditions} holds then
    \begin{equation}
        \partial_x \hat u_-(0,s) - \partial_x \hat u_+(0,s) = (\lambda_-(s)+\lambda_+(s)) 2 \hat v_i(0,s)
        \label{eq:coupling-conditions-equivalence-proof}
    \end{equation}
    is true for both $\hat v_i = \hat v_-$ and $\hat v_i=\hat v_+$. Then, if the second equation of \eqref{eq:coupling-conditions} also holds, the left hand side of \eqref{eq:coupling-conditions-equivalence-proof} is zero. Since $Re(\lambda_-)>0$ and $Re(\lambda_+)>0$, necessarily $v_+$ and $v_-$ are null. Then using the definition of $v_\pm$ we obtain the conclusion.
\end{proof}

At the same time, the coupling conditions \eqref{eq:coupling-conditions} can be reformulated in multiple equivalent ways.  In particular, if instead one defines transmission conditions using linear operators $B_-$, $B_+$ as 
\begin{equation}
    \begin{split}
        B_-(u_-(0,\cdot)) = B_-(u_+(0,\cdot))  \\
        B_+(u_-(0,\cdot)) = B_+(u_+(0,\cdot))  \\
    \end{split}
    \quad \text{ in } ]0,T[
    \label{eq:abstract-bis}
\end{equation} 
instead of \eqref{eq:coupling-conditions}, to preserve the solution of the hybrid model it is enough to choose $B_-$ and $B_+$ such that their Laplace transforms satisfy 
\begin{equation}
    \begin{split}
        \widehat{B u_-(0,\cdot)}   &= 
        \partial_x \widehat{u}_-
        + m_- \hat u_- + c_- \\ 
        \widehat{B u_+(0,\cdot)}   &= 
        \partial_x \widehat{u}_+
        + m_+ \hat u_+ + c_+         
    \end{split}
    \quad \text{ in } \mathbb{C}^+
    \label{eq:coupling-conditions-equivalence}
\end{equation}
with $m_\pm(s), c_\pm(s): \mathbb{C}^+ \to \mathbb{C}$ such that $m_- - m_+ \neq 0$, which is the condition for equations \eqref{eq:abstract-bis} to be linearly independent in the frequency domain of the Laplace transform. This "trick" was noted by \cite{lions1990schwarz} in the context of domain decomposition methods and nowadays is commonly used to define optimized Schwarz methods \cite{gander2006optimized}.



\subsection{Well-posedness and coupling error}
\label{sec:coupling-error}
In this section we focus on the derivation of an explicit solution of \eqref{eq:hybrid-compact} in the case where $\vect W_0$ is supported in one of the subdomains. For simplicity we will assume that $supp(\vect W_0) \subset \Omega_-$ and that either $\mathcal{L}_- = \mathcal{L}_B$ and $\mathcal{L}_+=\mathcal{L}_{SV}$, the BSV case, or $\mathcal{L}_- = \mathcal{L}_{SV}$ and $\mathcal{L}_+=\mathcal{L}_{B}$, the SVB case. We will denote by $(\lambda_-(s), \vect v_1^-, \vect v_2^-)$ and $(\lambda_+(s), \vect v_1^+, \vect v_2^+)$ the positive eigenvalue and pair of eigenvectors of the diagonalization \eqref{eq:halfline-diagonalization}, for  $\mathcal{L}_-$ and $\mathcal{L}_+$ respectively, which is valid for both $\mu=0$ and $\mu>0$.

The idea is to use these assumptions to write the solution $\vect W$ as 
\begin{equation}
    \begin{split}
        \vect W = \vect W^\star+ \vect W' & \quad \text{ in } Q
        \label{eq:exact-solution-abstract}
    \end{split}
\end{equation}
where $\vect W'$ is an unknown perturbation of $\vect W^\star$, the solution to the one-way coupling, given by
\begin{equation}
    \vect W^\star = \left\{ 
    \begin{array}{cc}
        \vect W_{cauchy,-} & \text{ in } Q_- \\ 
        \vect W_{half,+} & \text{ in } Q_+
    \end{array}
    \right.
\end{equation} 
with $\vect W_{cauchy,-}$ and $\vect W_{half,+}$ the solutions to the Cauchy and half-line problems 
\begin{equation}
    \left\{ 
        \begin{array}{cc}
            \mathcal{L}_{-} \vect W_{cauchy,-} =0, & \quad \text{ in } Q\\ 
            \vect W_{cauchy,-} (\cdot, 0) = \vect W_0 & \quad \text{ in } \Omega
        \end{array}
    \right.
\end{equation}
and
\begin{equation} 
    \left\{ 
        \begin{array}{cc}
            \mathcal{L}_{+} \vect W_{half,+} =0, & \quad \text{ in } Q_+ \\ 
            \vect W_{half,+}(\cdot, 0) = 0 & \quad \text{ in } \Omega_+ \\ 
            u_{half,+}(0,\cdot) = u_{cauchy,-}(0,\cdot) & \quad \text{ on } ]0,T[
        \end{array}
    \right., 
\end{equation}

By definition  $\vect W'$ is unknown and will be obtained using Laplace-transform formulas and a reflection method. This method is similar to the one used in the study of one-dimensional IBVPs of the 1D wave equation \cite{evans1988}, except that in this case the amplitude of the reflection, the reflection coefficient, depends on the frequency, \textit{i.e.}, it is a filter. Such a reflection coefficient has also been derived in the study of absorbing boundary conditions \cite{engquist1979rad,engquist1977,GIVOLI2004319, Halpern1982}.  But so far, to the authors' knowledge, this is the first time it is used to study the coupling of wave equations with different dispersion relations. 


In the following we start by deriving the reflection coefficient using another choice of transmission conditions equivalent to \eqref{eq:coupling-conditions}. Then, we use the reflection method to analyze $\vect W'$, distinguishing the cases $\mathcal{L}_-= \mathcal{L}_B$ and $\mathcal{L}_-=\mathcal{L}_{SV}$.

\subsubsection{Coupling error and the reflection coefficient}

To derive the solution for the perturbation $\vect W'$ we will use the transmission conditions 
\begin{equation}
    \left\{ \begin{array}{rll}
        (\partial_x  + \lambda_+) \hat u_-(0,\cdot) 
        &= (\partial_x  + \lambda_+ )\hat u_+(0,\cdot) 
          &
        \quad \text{ in } \mathbb{C}^+ \\ 
        u_+(0,\cdot) 
        &= u_-(0,\cdot)  
        &\quad \text{ in } ]0,T[
    \end{array}\right.
    \label{eq:solution-transmission-conditions}
\end{equation}
which satisfy \eqref{eq:coupling-conditions-equivalence}, so they are equivalent to \eqref{eq:coupling-conditions} and by Theorem \eqref{th:hybrid-coupling-conditions} the solution of \eqref{eq:hybrid-halflines} will be the same as the solution of the hybrid model. Moreover, because $supp(\vect W_0)\subset \Omega_-$, using the results and notations of the half line problems of \Cref{ch:half-line}, $\vect W_+$ satisfies 
\begin{equation}
    \vect{\widehat W}_+(x,s) = \hat u(0,s) \vect v_1^+ e^{-\lambda_+(s)x},\quad (x,s) \in \Omega_+\times \mathbb{C}^+
\end{equation}
and the right hand side of the first line of equation \eqref{eq:solution-transmission-conditions} is 
\begin{equation}
    (\partial_x  + \lambda_+ )\hat u_+(0,\cdot)  = 0 
\end{equation}
which is the exact absorbing boundary condition of the operator $\mathcal{L}_+$. In the BSV the operator is local and corresponds to the transport operator
\begin{equation}
    (\partial_t + \partial_x)u_-(0,\cdot) = 0 
\end{equation}
while in the SVB case it is a pseudo-differential operator and was described in \cite{kazakova2020discrete}.


Because of \eqref{eq:solution-transmission-conditions}, denoting $\vect W_-'=(\eta_-',u_-') = \vect W_- - \vect W^{\star}_{cauchy,-}$ :
\begin{equation}
    (\partial_x + \lambda_+) \hat u_-'(0,\cdot)= -(\partial_x + \lambda_+) \hat{ u}^{\star}_{cauchy,-}(0,\cdot) \quad \text{, in } \mathbb{C}^+
    \label{eq:transmission-conditions-perturbation}
\end{equation}
and because $\hat{u}^{\star}_{cauchy,-}$ also satisfies the half-line problem \eqref{eq:half-line-solution} in $Q_+$ with trace $u^\star_{cauchy,-}(\cdot,)$, we have that
\begin{equation}
    \begin{array}{rll}
        \partial_x \widehat{u}^{\star}_{cauchy,-} 
            &= -\lambda_- \widehat{u}^{\star}_{cauchy,-} 
            & \text{ in } \overline{\Omega_+} \times \mathbb{C}^+ \\ 
        \partial_x \widehat u'_- 
        &= \lambda_- \widehat u'_- 
        & \text{ in } \overline{\Omega_-} \times \mathbb{C}^+ 
    \end{array}
\end{equation}
substituting into \eqref{eq:transmission-conditions-perturbation} we obtain that
\begin{equation}
    \hat u_-'(0,s) = r(s) \widehat{u}^{\star}_{cauchy,-}(0,s) \quad s \in \mathbb{C}^+ \quad \text{ with }\quad  r(s) = \frac{\lambda_-(s)-\lambda_+(s)}{\lambda_-(s)+\lambda_+(s)}
    \label{eq:reflection-coefficient-appearance}
\end{equation}
from \eqref{eq:reflection-coefficient-appearance} we can obtain $\vect W_-'$ and $\vect W_+'$ from the propagation of the signal 
\begin{equation}
    u_\Gamma = \mathcal{L}^{-1}(r \hat u^\star_{cauchy,-}(0,\cdot) ) \quad \text{ in }]-,T[
\end{equation}
on each half-line problem \eqref{eq:half-line-problem}, however, a more expressive formula can be obtained. Using \eqref{eq:half-line-solution} for $\vect W_-'$ and $\vect{W}^{\star}_{cauchy,-}$, we know that
\begin{equation}
    \begin{array}{rll}
        \vect{\widehat W}_-'(x,s) 
        &= r(s) \widehat{ u}^{\star}_{cauchy,-}(0,s) \vect v_2^- e^{\lambda_-(s)x} \quad 
        & \text{ in } \Omega_- \times \mathbb{C}^+ \\ 
        \vect{\widehat{W}}^{\star}_{cauchy,-}(x,s) 
        &=  \widehat{ u}^{\star}_{cauchy,-}(0,s) \vect v_1^- e^{-\lambda_-(s)x} \quad 
        & \text{ in } \Omega_+ \times \mathbb{C}^+
    \end{array}
    \label{eq:reflection-laplace-interm-formulas}
\end{equation}
and since 
\begin{equation}
    \vect v_2^- = G \vect v_1^- \quad \text{ with } G = \left(\begin{array}{cc}
        -1 & 0 \\
        0 & 1
    \end{array}\right)
    \label{eq:g-definition}
\end{equation}
we obtain
\begin{equation}
    \vect{\widehat W}_-'(x,s) = r(s) G \vect{\widehat{ W}}^{\star}_{cauchy,-}(-x,s) \quad \text{ in } \overline{\Omega}_- \times \mathbb{C}^+
    \label{eq:reflection-omega1-laplace}
\end{equation}
This expression shows already that the perturbation of the one-way coupling solution can be described by reflecting $\vect W_{cauchy,-}^\star$ through the $x$ axis and by filtering the solution in time by $r(s)$. This is why we refer to $\vect W_\pm'$ as reflections, even though $\vect W_+'$ is in the opposite direction. The formulation \eqref{eq:reflection-omega1-laplace} of the reflections may seem (anti) symmetric because $r(s)$ in \eqref{eq:reflection-coefficient-appearance} only changes sign when $\mathcal{L}_-$ is $\mathcal{L}_B$ or $\mathcal{L}_{SV}$. By using a reflection technique similar to the one sometimes used for the 1D wave equation \cite{evans1988}, the following sections show a more explicit representation that reveals the differences between these two cases.
\begin{remark}
    The reflection coefficient could be derived in the BSV case by noticing that \eqref{eq:solution-transmission-conditions} can be written as 
    \begin{equation}
        (\partial_t + \partial_x)u_-(0,\cdot) = 0 
    \end{equation}
    so, following a classical procedure on absorbing boundary conditions \cite{engquist1977,engquist1979rad,Halpern1982} one can replace $u_-(x,t) = e^{j (\kappa x - \omega(\kappa)t)}+r(\kappa)e^{j (-\kappa x - \omega(\kappa)t)}$, with $\omega(\kappa)$ the dispersion relation of the Boussinesq model, evaluate at $x=0$ and obtain
    \begin{equation}
        r(\kappa) = \frac{\sqrt{1+\mu^2\kappa^2}-1}{\sqrt{1+\mu^2\kappa^2}+1}
    \end{equation}
    which coincides with one of the formulas of  \Cref{sec:numerical-reflections}. However, in the SVB case, the transparent boundary condition \eqref{eq:solution-transmission-conditions} is a nonlocal pseudo-differential operator \cite{kazakova2020discrete}, and the application of this simple method is not clear. With the current derivation, not only this case can be handled, but also a precise analysis of the model can be derived for arbitrary initial data, which is not possible with the more classical approach.
\end{remark}


\subsubsection{Boussinesq to Saint-Venant case}
We start with the case $\mathcal{L}_- = \mathcal{L}_{B}$ and $\mathcal{L}_+ = \mathcal{L}_{SV}$ (BSV) using the dispersion relation in \eqref{eq:dispersion-relation} that will denoted by $\omega_-(\kappa)$. In the next \Cref{th:b-reflection} the Taylor expansion of $r(s)$  with convergence region $|\mu s|<1$ 
\begin{equation}
    r_N(s) = \sum_{n=1}^N a_n (\mu s)^{2n}
    \label{eq:truncated-coefficient}
\end{equation}
will simplify the inversion of \eqref{eq:reflection-omega1-laplace} and reformulate $\vect W_-'$ as the solution of a Cauchy problem.
\begin{theorem}
    \label{th:b-reflection}
    Let $\mathcal{L}_-=\mathcal{L}_B$. If $\vect W_0$ is supported on $\Omega_-$ then $\vect{\widehat W}_-'$ is the restriction to $\Omega_-$ of the solution of the Cauchy problem  
    \begin{equation}
        \left\{\begin{array}{cc}
            \mathcal{L}_{B} \vect W = 0 & \text{ in } Q \\
            \vect W(0, \cdot) = \mathcal{F}^{-1}\left(r(j\omega_-)\right) * G R \vect W_0   & \text{ in }  \Omega
        \end{array}\right.
    \end{equation}    
    where $R$ is such that $Rf(x) = f(-x)$ and $\mathcal{F}^{-1}$ is the inverse Fourier transform.
\end{theorem}

\begin{proof}
    Let $ \vect{\widehat W}^N$ be such that 
    \begin{equation}
        \widehat{\vect W}^N(x,s) = r_N(s) G \vect{\widehat{ W}}^\star_-(-x,s) \quad x \in \Omega_-
    \end{equation}
    taking the inverse Laplace transform this means that 
    \begin{equation}
        \vect W_-^N(x,t) = \mathcal{L}^{-1}(r_N(s) )* G \vect{ W}^\star_-(-x,\cdot)
    \end{equation}
    since it is a finite sum, we can write 
    \begin{equation}
        \mathcal{L}^{-1}(r_N(s)) * f = \sum_{n=1}^N a_n \mu^{2n} \partial_t^{2n}f 
    \end{equation}
    also, from  \eqref{eq:lgn-homogeneous-cauchy-fourier-solution} 
    \begin{equation}
        \vect{W}(-x,t) = \int_\mathbb{R} e^{j\kappa x} S^{-1}e^{Jt} S \widehat{\vect W}_0(-\kappa) d\kappa
    \end{equation}    
    which means that
    \begin{equation}
        \begin{split}
            \vect{W}_-^N(x,t) &= \mathcal{L}^{-1}(r_N(s) )* G \vect{ W}^\star_-(-x,\cdot) \\ 
            &= \sum_{n=1}^N a_n \mu^{2n}\partial_t^{2n} G \vect{ W}^\star_-(-x,\cdot)\\
            &= \int_\mathbb{R}\sum_{n=1}^N a_n \mu^{2n}  e^{j\kappa x} S^{-1}\partial_t^{2n}\left(e^{Jt}\right) S G \widehat{\vect W}_0(-\kappa) d\kappa
        \end{split}
    \end{equation}
    and since 
    \begin{equation}
        \partial_t^{2n} e^{Jt} = (j \omega_-(\kappa))^{2n} e^{Jt}
    \end{equation}
    after rearranging one can substitute the definition of $r_N$ as
    \begin{equation}
        \begin{split}
            \vect{W}_-^N(x,t) &= \int_\mathbb{R}  e^{j\kappa x} S^{-1}e^{Jt} S \left(\sum_{n=1}^N a_n (\mu j\omega)^{2n} G \widehat{\vect W}_0(-\kappa)\right) d\kappa \\ 
            &= \int_\mathbb{R}  e^{j\kappa x} S^{-1}e^{Jt} S \left(r_N(j\omega) G \widehat{\vect W}_0(-\kappa)\right) d\kappa             
        \end{split}
    \end{equation}   
    since $\mu|\omega(\kappa)|<1$ we can take the limit $N \to \infty$ to obtain
    \begin{equation}
        \vect{W}_-'(x,t) = \int_\mathbb{R}  e^{j\kappa x} S^{-1}e^{Jt} S \left(r(j\omega) G \widehat{\vect W}_0(-\kappa)\right) d\kappa
    \end{equation}
    and comparing with \eqref{eq:lgn-homogeneous-cauchy-fourier-solution} we conclude that $\vect W_-'$ is the solution of \eqref{eq:lgn-homogeneous-cauchy} with initial condition $\mathcal{F}^{-1}\left(r(j\omega)  \right) * G R \vect W_0$.
\end{proof}



\subsubsection{Saint-Venant to Boussinesq case}

The key argument for the convergence of the integrals involved in the proof of \Cref{th:b-reflection} is that the dispersion relation satisfies $\mu |\omega|<1$, so the Taylor series converges. Under this assumption one can repeat the same argument \eqref{th:b-reflection} to obtain that

\begin{proposition}
    If $\mathcal{L}_-=\mathcal{L}_{SV}$, $\vect W_0$ is supported on $\Omega_-$ and $\mathcal{F}(\vect{W}_0)$ is supported on $]-\dfrac{1}{\mu},\dfrac{1}{\mu}[$, then $\vect{ W}_-$ is the restriction to $\overline{\Omega}_-$ of the solution of he Cauchy problem  
    \begin{equation}
        \left\{\begin{array}{cc}
            \mathcal{L}_{SV} \vect W = 0 & \text{ in } Q \\
            \vect W(0, \cdot ) = \mathcal{F}^{-1}\left(r(j\omega_-)\right) * G R \vect W_0    & \text{ in }  \Omega
        \end{array}\right.
    \end{equation}    
\end{proposition}
The assumption on the spectrum is too strong, however, using formula \eqref{eq:sv-cauchy-solution} and the assumption on the support of the initial data one obtains the following:

\begin{theorem}
    \label{th:sv-reflection}
    If $\mathcal{L}_-=\mathcal{L}_{SV}$, $\vect W_0$ is supported on $\Omega_-$ then $\vect{ W_-}'=(\eta_-', u_-')$ is the restriction to $\overline{\Omega_-}$ of the solution $\vect W=(\eta,u)$ of the Cauchy problem  
    \begin{equation}
        \left\{\begin{array}{cc}
            \mathcal{L}_{SV} \vect W = 0 & \text{ in } Q \\
            \vect W(0,\cdot) = H(x) \mathcal{L}^{-1}(r) * G R \vect W_0 & \text{ in } \Omega 
        \end{array}\right.
    \end{equation}    
\end{theorem}

\begin{proof}
    From \eqref{eq:sv-cauchy-solution}, because $\vect W_0 =0$ in $Q_+$
\begin{equation}
    {u}^\star_{cauchy,-}(0,t) = \frac{1}{2}(\eta_0+u_0)(-t) \quad t\geq 0
\end{equation}
substituting on the first equation of \eqref{eq:reflection-laplace-interm-formulas} we obtain 
\begin{equation}
    \vect{\widehat W}_-'(x,s)=\frac{r(s)}{2} (\widehat{R\eta_0}(s) + \widehat{Ru_0}(s)) \left( \begin{array}{c}
        -1 \\
        1
    \end{array}\right) e^{sx}
\end{equation}
so taking the inverse Laplace transform  
\begin{equation}
    \begin{split}
        \eta_-'(x,t) = - \mathcal{L}^{-1}\left(\frac{r}{2} (\widehat{R\eta_0} + \widehat{Ru_0}) \right) ( t+x) H(t+x)  \\ 
        u_-'(x,t) = \mathcal{L}^{-1}\left(\frac{r}{2} (\widehat{R\eta_0} + \widehat{Ru_0}) \right) ( t+x) H(t+x) 
    \end{split}
    ,\quad \text{ in } \Omega_-
\end{equation}
if we now denote $\tilde \eta_0(x) =  - \mathcal{L}^{-1}(r \widehat{R\eta_0} )$ and $\tilde u_0(x) =  \mathcal{L}^{-1}(r \widehat{R u_0})$ then 
\begin{equation}
    \begin{split}
        \eta_-'(x,t) &= \frac{1}{2}(\tilde \eta_0(x+t) - \tilde u_0(x+t))\\ 
        u_-'(x,t) &= -\frac{1}{2}(\tilde \eta_0(x+t) - \tilde u_0(x+t))
    \end{split}
\end{equation}
which contrasted with \eqref{eq:sv-cauchy-solution} proves the conclusion.
\end{proof}


\subsubsection{Well-posedness}
Because $\vect W_- = \vect W^\star_{cauchy,-} + \vect W'_-$ we can leverage our knowledge that both $\vect W^\star_{cauchy,-}$ and $\vect W'_-$ solve a Cauchy problem that depends on $\vect W_0$ to prove that the hybrid model depends continuously on the initial data. This result can later be extended to data not necessarily contained on one side of the interface by means of a density argument. To simplify the notation, in the following we will denote 
\begin{equation}
    a \lesssim b
\end{equation}
to say that there exists a constant $C>0$ such that $a \leq C b$.

\begin{proposition}
    \label{th:continuity-one-side}
    Let $n \geq 0$, $\vect W_0 \in H^{n+1}(\Omega)\times H^{n+1}(\Omega)$ with $supp(\vect W_0) \subset \mathbb{R}^{-}$ and $\vect W$ the solution of the hybrid model. There exists a constant $C>0$ such that 
    \begin{equation}
        |\vect W|_{(H^{n,n}(Q))^2} \leq C |\vect W_0|_{H^{n+1}\times H^{n+1}(\Omega)}
    \end{equation}
\end{proposition}
\begin{proof}
    \emph{B to SV case:}
    Let $\mathcal{L}_- = \mathcal{L}_{B}$ and $\mathcal{L}_{+}=\mathcal{L}_{SV}$ and $\vect W_- = \vect W_{|Q_-}$ and $\vect W_+ = \vect W_{|Q_+}$. From \eqref{eq:exact-solution-abstract} we have $\vect W_- = \vect W^\star_{cauchy,-} + \vect W'_-$, so using \Cref{th:b-reflection} we deduce that $\vect W_-$ is solution of the Cauchy problem \eqref{eq:lgn-homogeneous-cauchy} with initial condition $\vect W_0^-$ given by 
    \begin{equation}
        \mathcal{F}(\vect W_0^-) =  (I + rGR)\mathcal{F}(\vect W_0), \quad 
    \end{equation}
    hence, using that $|r|\leq 1$ and \Cref{th:cauchy-b}
    \begin{equation}
        \begin{split}
            |\vect W_-|_{H^{n,s}(Q_-)\times H^{n,s}(Q_-)} &\lesssim |\vect W_0^-|_{H^{n+1}(\Omega_-)\times H^{n+1}(\Omega_-)} \\
            & \leq |\vect W_0 |_{H^{n+1}(\Omega)\times H^{n+1}(\Omega)}
        \end{split}, \quad \forall s \geq 0
    \end{equation}
    and $u_-' \in H^{n+1,s}(Q_-)$ so from \Cref{th:trace} $u_-(0,\cdot) \in H^{\nu_0}$ with $\nu_0 = s \dfrac{n+1/2}{n+1}$. Choosing $s$ such that $\nu_0 = n$ then from \Cref{th:halfline-sv} and the continuity of the trace in \Cref{th:trace}
    \begin{equation}
        \begin{split}
            |\vect W_+|_{(H^{n,n}(Q_+))^2} &\lesssim |u_-(0,\cdot)|_{H^n} \\ 
            &\lesssim |\vect W_-|_{H^{n,n}(Q_-)\times H^{n,n}(Q_-)} \\ 
            &\lesssim |\vect W_0|_{H^{n+1}(\Omega)\times H^{n+1}(\Omega)}
        \end{split}
    \end{equation}
    hence reconstructing the solution we obtain 
    \begin{equation}
        |\vect W|_{(H^{n,n}(Q))^2}  \lesssim |\vect W_0|_{(H^{n+1}(\Omega))^2}
    \end{equation}

    \emph{SV to B case:}
    Let now $\mathcal{L}_- = \mathcal{L}_{SV}$ and $\mathcal{L}_{+}=\mathcal{L}_{B}$. From \Cref{th:sv-reflection}, $\vect W_-$ is the solution of the Cauchy problem \eqref{eq:sv-cauchy} with initial condition $\vect W_0^-$ given by
    \begin{equation}
        \mathcal{L}(\vect W_0^-) =  (I + rGR)\mathcal{L}(\vect W_0)
    \end{equation}
    hence, using the \Cref{th:sv-cauchy}  and $|r|\leq 1$ 
    \begin{equation}
        \begin{split}
            |\vect W_-|_{(H^{m,m}(Q_-))^2} &\lesssim |\vect W_0^-|_{H^{m}(\Omega_-)\times H^{m}(\Omega_-)} \\
            & \lesssim |\vect W_0 |_{H^{m}(\Omega)\times H^{m}(\Omega)}
        \end{split}
    \end{equation}
    also $u_-' \in H^{m,m}(Q_-)$ and $u_-(0,\cdot) \in H^{m}(0,T)$. Then, from \Cref{th:halfplane-boussinesq} and the continuity of the trace w.r.t the initial data (which can be derived from \eqref{eq:sv-cauchy-solution})
    \begin{equation}
        \begin{split}
            |\vect W_+|_{H^{r,m+1}(Q_+)\times H^{r,m}(Q_+)} &\lesssim |u_-(0,\cdot)|_{H^{m}} \\ 
            &\lesssim |\vect W_0^-|_{(H^{m}(\Omega_-))^2} \\ 
            &\lesssim |\vect W_0|_{(H^{m}(\Omega))^2} \\
        \end{split}
    \end{equation}
    Taking $r=m$ and reconstructing $\vect W|_{Q_-} = \vect W_-$ and $\vect W_{Q_+}=\vect W_+$ 
    \begin{equation}
        |\vect W|_{(H^{m,m}(\Omega))^2}  \lesssim |\vect W_0|_{H^{m}(\Omega)\times H^{m}(\Omega)}
    \end{equation}
    and taking $m=n+1$ this implies 
    \begin{equation}
        |\vect W|_{(H^{n,n}(Q))^2}  \lesssim |\vect W_0|_{(H^{n+1}(\Omega))^2}
    \end{equation}
\end{proof}
\begin{proposition}
    Let $n\geq 0$, if $\vect W_0 \in H^{n+1}(\Omega)\times H^{n+1}(\Omega)$ and $\vect W$ is the solution of the hybrid model, then there exists a constant $C>0$ such that 
    \begin{equation}
        |\vect W|_{(H^{n,n}(Q))^2} \leq C |\vect W_0|_{H^{n+1}\times H^{n+1}(\Omega)}
    \end{equation}
\end{proposition}
\begin{proof}
    The proof will be done by a density argument. Let $\vect W \in M\times M$, with 
    \begin{equation}
        M = \{f \in C^\infty(\mathbb{R}) : \quad f(0) = 0)\}
    \end{equation}
    and let $\mathcal{T}_{0}$ such that 
    \begin{equation}
        \vect W = \mathcal{T}_0 \vect W_0 
    \end{equation}
    is the solution of hybrid's problem \eqref{eq:hybrid-compact}. Define 
    \begin{equation}
        \vect W_0^L = \left\{\begin{array}{cc}
            \vect W_0 & \quad \text{ in } \Omega_- \\ 
             0 & \quad \text{ in } \Omega_+ 
        \end{array} \right.,\quad 
        \vect W_0^R = \left\{\begin{array}{cc}
             0  & \quad \text{ in } \Omega_- \\ 
            \vect W_0 & \quad \text{ in } \Omega_+ 
        \end{array} \right.,
        \label{eq:w0-splitting}
    \end{equation}
    then from \Cref{th:continuity-one-side}
    \begin{equation}
        |\mathcal{T}_0 \vect W_0^L |_{(H^{n,n}(Q))^2} \lesssim |\vect W_0^L|_{(H^{n+1}(\Omega))^2}
    \end{equation}
    \begin{equation}
        |\mathcal{T}_0 \vect W_0^R |_{(H^{n,n}(Q))^2} \lesssim |\vect W_0^R|_{(H^{n+1}(\Omega))^2}
    \end{equation}
    and by linearity
    \begin{equation}
        |\mathcal{T}_0 \vect W_0 |_{(H^{n,n}(Q))^2} \lesssim |\vect W_0|_{(H^{n+1}(\Omega))^2}
    \end{equation}
    which means that $\mathcal{T}_0$ is a linear bounded operator from $(C^\infty_0(\mathbb{R}))^2 \subset (H^{n+1}(\Omega))^2$ to $(H^{n,n}(Q))^2$. From \Cref{th:M0-dense-L2} we deduce that $(C^\infty_0(\mathbb{R}))^2$ is dense in $(H^{n+1}(\Omega))^2$ which, due to \Cref{th:unique-extension}, means that there exists a unique continuous operator 
    \begin{equation}
        \begin{array}{lll}
            \mathcal{T}:& (H^{n+1}(\Omega))^2 &\to (H^{n,n}(Q))^2\\
                & \vect W_0 & \to \vect W = \mathcal{T} \vect W_0
        \end{array}
    \end{equation}
    such that $\mathcal{T} \vect W_0 = \mathcal{T}_0 \vect W_0$ for every $\vect W_0 \in M$.    
\end{proof}
\subsubsection{Estimation of the coupling error}
As already stated, the size of the reflections $\vect W_\pm'$ is a measure of the error introduced by a particular coupling technique. In this section we study its asymptotic behavior as $\mu \to 0$.  For this, the following \Cref{th:trace-reflection-asymptotic-estimate} quantifies the asymptotic behavior of the trace of the reflections at $x=0$, which will facilitate the estimation of $\vect W'_\pm$.


\begin{lemma}
    \label{th:trace-reflection-asymptotic-estimate}
    Let $f \in H^{n+2}(\mathbb{R}^+)$ with $n \geq 0$ integer, there exits $C>0$ such that
    \begin{equation}
        |\mathcal{L}^{-1}(r) * f |_{H^{n}(\mathbb{R}^+)} \leq C \mu^2 |f|_{H^{n+2}(\mathbb{R}^-)}
    \end{equation}
\end{lemma}
\begin{proof}
    From Theorem \ref{eq:approx-theory} there exists a family of functions $(\hat f_h)_{h>0} \subset C_0^\infty(\mathbb{R})$, and positive constants $c_1, c_2$, such that 
    $$\hat f_h = \hat f \text{ in } \left( -\frac{c_1}{h},\frac{c_1}{h}\right) \subset supp(\hat f_h) = ( -\frac{c_2}{h}, \frac{c_2}{h})$$ and
    \begin{equation}
            |\hat f - \hat f_h|_{H^{n}(\mathbb{R})} \leq C_1 h |\hat f|_{H^{n+1}(\mathbb{R})}
            \label{eq:bound-for-fh}
    \end{equation}
    so we can compute 
    \begin{equation}
        \begin{split}
            |r \hat f|_{H^{n}(\mathbb{R})}^2 &\leq |r(\hat f-\hat f_h)|^2_{H^n(\mathbb{R})} + |r \hat f_h|^2_{H^n(\mathbb{R})}\\
            &= \int_\mathbb{R} (1+\omega^2)^n|r|^2 |\hat f -\hat f_h|^2 d\omega + \int_\mathbb{R} (1+\omega^2)^n |r|^2 |\hat f_h|^2 d\omega \\ 
            & =\int_{|\omega|\geq \frac{c_1}{h}} (1+\omega^2)^n|r|^2 |\hat f - \hat f_h|^2 d\omega  + \int_{|\omega| \leq \frac{c_2}{h}} (1+\omega^2)^n|r|^2 |\hat f_h|^2 d\omega \\ 
        \end{split}
    \end{equation}
    where the limit of the first integral is obtained from the region where $\hat f = \hat f_h$, and the limit of the second integral from the support of $\hat f_h$. Since $|r| \leq 1$, we can proceed to use \eqref{eq:bound-for-fh} to obtain 
    \begin{equation}
        |r \hat f|_{H^n(\mathbb{R})}^2 \leq C_1^2 h^2 |\hat f|_{H^{n+1}(\mathbb{R})}^2 + \int_{|\omega| \leq \frac{c}{h}} |r|^2 |\hat f_h|^2 d\omega
    \end{equation}
    Since we have
    \begin{equation}
        r(s) = -\frac{1}{4}\mu^2 s^2 + O(|\mu s|^4) \quad \text{ if } |\mu s| \leq  c' < 1
    \end{equation}
    then choosing $h = \dfrac{c}{c'} \mu^2$ and $\sigma$ very small, developing the integral one obtains that there exists $C_2>0$ such that 
    \begin{equation}
        \int_{|\omega| \leq \frac{c}{h}} |r|^2 |\hat f_h|^2 d\omega \leq C_2 \mu^4 |f_h|_{H^{n+2}}
    \end{equation}
    from where we deduce that there exists $C_3$ such that 
    
    \begin{equation}
        |\mathcal{L}^{-1} (r) * f|_{H^n(\mathbb{R}^+)}^2 \leq \mu^4  C_3 |f_h|_{H^{n+2}(\mathbb{R}^+)}^2
    \end{equation}
\end{proof}

The next \Cref{th:asymptotic-size-of-reflections-onesided} shows that as $\mu\to 0$ the size of the coupling error  $\vect W_\pm'$, \textit{i.e.}, the reflections, is $O(\mu^2)$.

\begin{proposition}
    \label{th:asymptotic-size-of-reflections-onesided}
    Let $\vect W_0 \in (H^n(\Omega))^2$ and $supp(\vect W_0)\subset \Omega_-$, for every $r, k > 0 $ there exists $C(r,k)>0$ and $C>0$ such that  if $\mathcal{L}_- =\mathcal{L}_{B}$ then 
    \begin{equation}
        \begin{split}
            |\vect W_-'|_{H^{r,k+1}(Q_-)\times H^{r,k}(Q_-)} \leq C(r,k) \mu^2 |\vect W_0|_{(H^n(\Omega))^2} \\ 
            |\vect W_+'|_{H^{k,k}(Q_+)\times H^{k,k}(Q_+)} \leq C(r,k) \mu^2 |\vect W_0|_{(H^n(\Omega))^2} \\ 
        \end{split}
    \end{equation}
    and if $\mathcal{L}_-  = \mathcal{L}_{SV}$ then there is $C_1>0$ and $C_2(r)>0$ such that 
    \begin{equation}
        \begin{split}
            |\vect W_-'|_{H^{n,n}(Q_-)\times H^{n,n}(Q_-)} \leq C_1 \mu^2 |\vect W_0|_{(H^{n+2}(\Omega))^2} \\ 
            |\vect W_+'|_{H^{r,n+1}(Q_+)\times H^{r,n}(Q_+)} \leq C_2(r) \mu^2 |\vect W_0|_{(H^{n+2}(\Omega))^2} \\ 
        \end{split}
    \end{equation}
\end{proposition}
\begin{proof}
    Suppose $\mathcal{L}_- = \mathcal{L}_B$ then for all $r \geq 0$ and $k\geq 0$
    \begin{equation}
        \begin{split}
            |\vect W_-'|_{H^{r,k+1}(Q_-)\times H^{r,k}(Q_-)} &\lesssim |u_-'(0,\cdot)|_{H^k}(0,T)  \quad \text{(\Cref{th:halfplane-boussinesq})}\\ 
            &\lesssim C \mu^2 |u^\star_{cauchy,-}(0,\cdot)|_{H^{k+2}(0,T)} \quad \text{(\Cref{th:trace-reflection-asymptotic-estimate})} \\ 
            &\lesssim C \mu^2 |\vect W_{cauchy,-}^\star|_{(H^{n,s_k}(Q))^2} \quad \text{(\Cref{th:trace})} \\ 
            &\lesssim \mu^2 | \vect W_0|_{(H^n(\Omega))^2} \quad \text{(\Cref{th:cauchy-b})}
        \end{split}
    \end{equation}
    with $s_k = (k+2)\frac{n+1}{n+1/2}$, thanks to the continuity of the trace in \Cref{th:trace}. Similarly
    \begin{equation}
        \begin{split}
            |\vect W_+'|_{H^{k,k}(Q_+)\times H^{k,k}(Q_+)} &\lesssim |u_-'(0,\cdot)|_{H^k}(0,T)  \quad \text{(\Cref{th:halfline-sv})}\\ 
            &\lesssim C \mu^2 |u^\star_{cauchy,-}(0,\cdot)|_{H^{k+2}((0,T))} \quad \text{(\Cref{th:trace-reflection-asymptotic-estimate})} \\ 
        &\lesssim C \mu^2 |\vect W_{cauchy,-}^\star|_{(H^{n,s_k}(Q))} \quad \text{(\Cref{th:trace})} \\ 
            &\lesssim \mu^2 | \vect W_0|_{(H^n(\Omega))^2} \quad \text{(\Cref{th:cauchy-b})}
        \end{split}
    \end{equation}
    Suppose now that $\mathcal{L}_- = \mathcal{L}_{B}$, then 
    \begin{equation}
        \begin{split}
            |\vect W_-'|_{H^{n,n}(Q_-)\times H^{n,n}(Q_-)} &\lesssim |u_-'(0,\cdot)|_{H^n}(0,T)  \quad (\text{\Cref{th:halfline-sv}})\\ 
            &\lesssim C \mu^2 |u^\star_{cauchy,-}(0,\cdot)|_{H^{n+2}(0,T)} \quad \text{(\Cref{th:trace-reflection-asymptotic-estimate})} \\ 
            &\lesssim C \mu^2 |\vect W_{cauchy,-}^\star|_{(H^{n+2,n+2}(Q))^2} \quad \text{(\Cref{th:sv-cauchy})} \\ 
            &\lesssim \mu^2 | \vect W_0|_{(H^{n+2}(\Omega))^2} \quad \text{(\Cref{th:cauchy-b})}
        \end{split}
    \end{equation}
    and for every $r \geq 0$
    \begin{equation}
        \begin{split}
            |\vect W_+'|_{H^{r,n+1}(Q_+)\times H^{r,n}(Q_+)} &\lesssim |u_-'(0,\cdot)|_{H^n(0,T)} \quad \text{ (\Cref{th:halfplane-boussinesq})}\\ 
            &\lesssim C \mu^2 |u^\star_{cauchy,-}(0,\cdot)|_{H^{n+2}(0,T)} \quad \text{(\Cref{th:trace-reflection-asymptotic-estimate})} \\ 
            &\lesssim C \mu^2 |\vect W_{cauchy,-}^\star|_{(H^{n+2,n+2}(Q))^2} \quad \text{(\Cref{th:trace})} \\ 
            &\lesssim \mu^2 | \vect W_0|_{(H^{n+2}(\Omega))^2} \quad \text{(\Cref{th:cauchy-b})}
        \end{split}
    \end{equation}    
\end{proof}
To generalize this result to the case of initial data with arbitrary support, let us define 
\begin{equation}
    \vect W^{\star\star\star}  = \vect W^\star_L  + \vect W^\star_R
\end{equation}
where $\vect W^\star_L$ is the solution of the one-way coupling \eqref{eq:one-way-model-right-moving} initialized with $\vect W_0^L$ as in \eqref{eq:w0-splitting}; and $\vect W^\star_R$ is the solution of the one-way coupling initialized with $\vect W_0^R$, but solved in the opposite direction, \textit{i.e.},
\begin{equation}
    \vect W^\star_R = \left\{ 
    \begin{array}{cc}
        \vect W_{half,-} & \text{ in } Q_- \\
        \vect W_{cauchy,+} & \text{ in } Q_+ \\ 
    \end{array}
    \right.
\end{equation} 
where
\begin{equation}
    \left\{ 
        \begin{array}{cc}
            \mathcal{L}_{+} \vect W_{cauchy,+} =0, & \quad \text{ in } Q_+ \\ 
            \vect W_{cauchy,+} (\cdot, 0) = \vect W_0^R & \quad \text{ in } \Omega_+
        \end{array}
    \right.
\end{equation}
and
\begin{equation} 
    \left\{ 
        \begin{array}{cc}
            \mathcal{L}_{-} \vect W_{half,-} =0, & \quad \text{ in } Q_- \\ 
            \vect W_{half,-}(\cdot, 0) = 0 & \quad \text{ in } \Omega_+ \\ 
            u_{half,-}(0,\cdot) = u_{cauchy,+}(0,\cdot) & \quad \text{ on } ]0,T[
        \end{array}
    \right., 
\end{equation}
so defining $\vect W' = \vect W - \vect W^{\star\star\star}$ one has the following result:

\begin{theorem}
    \label{th:asymptotic-size-of-reflections}
    Let $\vect W_0 \in H^{n+2}(\Omega) \times H^{n+2}(\Omega)$, there exists $C>0$ such that as $\mu$ goes to 0
    \begin{equation}
        |\vect W'|_{(H^{n,n}(\Omega))^2} \leq C \mu^2|\vect W_0|_{H^{n+2}(\Omega)\times H^{n+2}(\Omega)}
    \end{equation}
\end{theorem}
\begin{proof}
    Let 
    \begin{equation}
        M = \{f \in C^\infty(\mathbb{R}) : \quad f(0) = 0)\}
    \end{equation}
    and suppose $\vect W_0 \in M$. Also notice that 
     \begin{equation}
        \begin{split}
            \vect W' &=  \vect W - \vect W^{\star\star\star}  \\
            &= (\vect W_L - \vect W_L^\star) + (\vect W_R - \vect W_R^\star)
        \end{split}
    \end{equation}
    and from \Cref{th:asymptotic-size-of-reflections-onesided} one can deduce that 
    \begin{equation}
        |\vect W_L'|_{(H^{n,n}(Q))^2} \leq C \mu^2 |\vect W_0|_{H^{n+2}(\Omega)\times H^{n+2}(\Omega)}
    \end{equation}
    \begin{equation}
        |\vect W_R'|_{(H^{n,n}(Q))^2} \leq C \mu^2 |\vect W_0|_{H^{n+2}(\Omega)\times H^{n+2}(\Omega)}
    \end{equation}
    which means that 
    \begin{equation}
        |\vect W'|_{(H^{n,n}(Q))^2} \leq C \mu^2 |\vect W_0|_{H^{n+2}(\Omega)\times H^{n+2}(\Omega)}
        \label{eq:asymptotic-behavior}
    \end{equation}
    which means that the mapping 
    \begin{equation}
        \begin{array}{ll}
            \mathcal{T}'_0: M^2 &\to (H^{n,n}(Q))^2  \\ 
            \vect W_0 &\to \vect W'
        \end{array}
    \end{equation}
    is continuous, and because $M$ is dense in $H^{n+2}(\Omega)$ (\Cref{th:M0-dense-L2}) it has a unique extension  (\Cref{th:unique-extension})
    \begin{equation}
        \begin{array}{ll}
            \mathcal{T}': (H^{n+2}(\Omega))^2 &\to (H^{n,n}(Q))^2  \\ 
            \vect W_0 &\to \vect W'
        \end{array}
    \end{equation}
    and \eqref{eq:asymptotic-behavior} holds.
\end{proof}
\subsection{Numerical experiments}
\label{sec:numerical-reflections}
As we just saw, the reflections decrease as $O(\mu^2)$ in both cases (SVB and BSV), however, one can readily notice in \eqref{th:asymptotic-size-of-reflections-onesided} that when the wave propagates in the BSV case the regularity estimate of $\vect W'$ is much better than in the SVB case.

However, a more explicit explanation can be found by studying the filter $r(j\omega)$ that appears in both \eqref{th:b-reflection} and \eqref{th:sv-reflection}. For BSV and, in the limit $\sigma \to 0$ for SVB, these  filters take the form 
\begin{equation}
r_{BSV}(j\omega_1(\kappa)) = \dfrac{\sqrt{1+(\mu\kappa)^2}-1}{\sqrt{1+(\mu\kappa)^2}+1}    
\label{eq:bsv-filter}
\end{equation}
and 
\begin{equation}
    r_{SVB}(j\omega_1(\kappa))= \dfrac{1-\sqrt{1-(\mu\kappa)^2}}{1+\sqrt{1-(\mu\kappa)^2}}    
    \label{eq:wbt-filter}
\end{equation}
or changing to dimensional variables using \eqref{eq:dimensional-change}
\begin{equation}
    r_{BSV}(j\omega_1(\kappa)) = \dfrac{\sqrt{1+\frac{h_0^2}{3}\kappa^2}-1}{\sqrt{1+\frac{h_0^2}{3}\kappa^2}+1}    
\end{equation}
and 
\begin{equation}
    r_{SVB}(j\omega_1(\kappa))= \dfrac{1-\sqrt{1-\frac{h_0^2}{3}\kappa^2}}{1+\sqrt{1-\frac{h_0^2}{3}\kappa^2}}    
    \label{eq:wbt-filter-dimensional}
\end{equation}
One can already notice that $|r_{SVB}(\kappa)|$ and $|r_{BSV}(\kappa)|$ are increasing functions of $h_0|\kappa|$ and also that $|r_{SVB}(\kappa)|> |r_{BSV}(\kappa)|$. Morover, in the limit $h_0 |\kappa|\to \infty$ $|r_{SVB}| =|r_{BSV}| =1$ but $|r_{BSV}|<1$ for every $\kappa$, while $|r_{SVB}|=1$ for every $\frac{h_0^2}{3} \kappa^2>1$. This means that one should expect larger reflections in deeper waters and on SVB. These effects will be discussed with numerical examples in the next section, along with the study of the behavior when $\mu \to 0$.


\subsubsection{Discretization}
\label{eq:linear-discretization}
For the purpose of the discrete  hybrid model it is more convenient to write the equations  as
\begin{equation}
    \begin{split}
        \partial_t \eta + h \partial_x u &=0 \\ 
        \partial_t q + g \partial_x \eta &= 0 \\ 
        u - \dfrac{h_0^2}{3} \chi(x) \partial_{x}^2u &= q         
    \end{split}
\end{equation}
where we introduced the auxiliar variable $q$. Denoting by $H$ be the Heaviside function, $\chi$ will be either $H(x)$ or $1-H(x)$, depending on the case, and $g=9.81 m/s^2$. The discretization consists of a regular grid of sizes $(\Delta x, \Delta t)$ in space and time with nodes $(x_i)_{i=-2}^{n_x+3}$ and $(t_n)_{n=0}^{N}$, including 2 ghost cells on each side in $x$. Space derivatives are approximated  with the fourth-order centered finite differences:
\begin{equation}
    \begin{split}
        (\partial_x u)^n_{i} &= 
        \frac{1}{\Delta x}\left(
            \frac{1}{12} u^n_{i-2} - 
            \frac{2}{3}u^n_{i-1} + 
            \frac{2}{3} u^n_{i+1} - 
            \frac{1}{12} u^n_{i+2}\right) \\ 
        (\partial_x^2 u)^n_{i} &= 
        \frac{1}{\Delta x}\left(
            -\frac{1}{12} u^n_{i-2} - 
            \frac{4}{3} u^n_{i-1} -
            \frac{5}{2} u^n_i + 
            \frac{4}{3} u^n_{i+1} - 
            \frac{1}{12} u^n_{i+2}\right)       
    \end{split}
\end{equation}
where we denote $f(x_i,t_n)\approx f^n_i$. A third-order Runge-Kutta scheme is used in time, such that if we write the hybrid model as
\begin{equation}
    \partial_t \vect U = F(\eta, u, q)
\end{equation}
with $\vect U = (\eta, q)^T$ and $F(\eta,u,q) = (-h_0 \partial_x u, -g \partial_x \eta)^T$ then 
\begin{equation}
    \begin{split}
        \vect U^{(1)} &= \vect U^{n} + \Delta t F(\eta^n, u^n, q^n)\\ 
        \vect U^{(2)} &= \frac{3}{4} \vect U^{n} + \frac{1}{4} \vect U^{(1)} + \frac{1}{4}\Delta t F(\eta^{(1)}, u^{(1)}, q^{(1)}) \\ 
        \vect U^{n+1} &= \frac{1}{3}\vect U^{n} + \frac{2}{3} \vect U^{(2)} + \frac{2}{3} \Delta t F(\eta^{(2)}, u^{(2)}, q^{(2)})
    \end{split}
\end{equation}

Regarding the one-way model, $\vect W^\star_-$ is obtained using the previous scheme by setting $\chi(x)=1$ for $x\in\mathbb{R}$ or $0$ depending on the case (BSV or SVB resp.). For $\vect W^\star_+$, in the SVB case, the second line of equation \eqref{eq:half-line-solution} is discretized by approximating $\alpha_+(\sigma+j\omega)$ with the Fast Fourier Transform (FFT) of $e^{-\sigma t_n} u_{i\star}^n$, where $i\star$ is such that $\chi(x_{i\star})\neq \chi(x_{i\star+1})$. Also, $u_{i\star}^n$ is extended by 0 until $n=20N$ in order to improve the resolution in the frequency domain. The same strategy is used with $\mu=0$ to obtain $\vect W_+^\star$ in the  SVB  case, although the solution could be obtained from \eqref{eq:sv-halfline-solution-explicit} as well. 

\subsubsection{Initial conditions}
Two types of wave profiles are examined. The first is a smooth Gaussian wave
\begin{equation}
    \begin{split}
        \eta_0(x) &= 0 \\ 
        u_0(x) &= \frac{1}{\sqrt{2\pi \sigma^2}}e^{-\frac{1}{2} \frac{(x-x_0)^2}{\sigma^2}}
    \end{split}\quad x \in \mathbb{R} 
\end{equation}
with $\sigma=2/\sqrt{3}$ . The second type of wave profile is the rectangular wave
\begin{equation}
    \begin{split}
        \eta_0(x) &= 0 \\ 
        u_0(x) &= H(L-|x-x_0|)
    \end{split}\quad x \in \mathbb{R} 
\end{equation}
which is interesting as a proxy for the propagation of shock waves formed with the SV model in the nonlinear regime. These waves are compared in the deep water and shallow water cases with $h=4m$ and $h=1m$ respectively. In all cases the domain is truncated to $\Omega=(-200m,200m)$ which is large enough to avoid any influence from the boundaries. The mesh and timestep sizes are $\Delta x = 0.025 m$ and $\Delta t=  0.15 \Delta x/\sqrt{gh}$. 


\subsubsection{Results and discussion}

For the Gaussian wave, Figures \ref{fig:btsv-Gaussian-h1} and \ref{fig:btsv-Gaussian-h4} show the results at different times in the BSV case and Figures  \ref{fig:svbt-Gaussian-h1} and \ref{fig:svbt-Gaussian-h4} in the SVB case. In each figure the results of the hybrid and one-way coupled model, $u$ and $u^\star$, are shown first, followed by the numerical solution of  the problems describing the reflections  \Cref{th:b-reflection} and \Cref{th:sv-reflection}, shown in the graph as "filtered reflected Cauchy", along with the difference of the hybrid and the one-way coupling $u' = u-u^\star$. The discussion is only around the values of the velocity $u$, since for the surface elevation $\eta$ it is similar.

Furthermore, one can see that $u'$ and $u^\star_-$ coincide for every $x<0$, verifying the theory. Similarly, one can see that indeed the reflected wave decreases with the depth $h_0$ and that reflections are larger on SVB than on BSV, which is explained by the range of frequencies that are attenuated  by the reflection coefficient ($|r|<1$), which is only a compact interval in SVB, whereas it is the whole real line in BSV. Both facts, the decrease in size of the reflections with the depth and with BSV, can be verified by comparing the initial spectrum with the modulus of the reflection coefficients in \ref{fig:spectrum_vs_filter_svb} with \ref{fig:spectrum_vs_filter_bsv}. Besides the magnitude of the reflections alone, one can see that even in the case with the smallest reflections (shallow water and BSV, Fig. \ref{fig:btsv-Gaussian-h1}) the domain solving SV equations propagates the reflections more visibly. This can be explained by the fact that the phase speed of the SV equations is constant for all wave numbers, while it is close to 0 for large wave numbers in the Boussinesq equations.
Figures \ref{fig:SVBT-rect-h1} and \ref{fig:SVBT-rect-h4} show similar results with the rectangular initial wave profile. A similar conclusion can be obtained in this case, that is, the verification of the reflection's formula and the decrease in size with the depth. However, in this case the reflections are much larger even in the shallow-water case. As can be seen in Figures \ref{fig:spectrum_vs_filter_svb_rect} this can be explained by the fact that the spectrum of the initial condition decays as slow as $1/\kappa$, hence it is not compact, decreases slowly, so more harmonics are reflected. Notice also that high-frequency harmonics, both from reflections and from the square wave, are smoothed by the Boussinesq model. This can be explained by the  dispersive boundary layer explained in \Cref{sec:dispersive-layer}, that filters out frequencies not allowed in the dispersion relation, \textit{i.e.}, whose temporal variations have frequencies $|\omega|>\sqrt{gh}/\mu$, with $\mu = h_0/\sqrt{3}$. Current results have lots of numerical dispersion, but even those spurious waves are filtered out by the Boussinesq model.

Table \ref{table:empirical-convergence-reflections} shows the empirical convergence order $p$ obtained from computing the $L^2$ difference $u-u^\star$ at $x=0$, and fitting the curve $c \mu^p$ with a linear regression in the log-log plane. The results are computed for the Gaussian and rectangular initial conditions varying $h_0$ between $10^{-6}$ and $10^-2$ such that $\log(h_0)$ has a uniform spacing of $0.5$. This is done for both $SVB$ and $BSV$ cases. The results show a good agreement with the theoretical result $O(\mu^2)$ of \Cref{th:asymptotic-size-of-reflections}. 


\begin{table}[]
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Initial condition} & \textbf{Case} & \textbf{Order $O(\mu^p)$} \\ \hline
    Gaussian                   & BSV           & 1.996                     \\ \hline
                               & SVB           & 2.000                     \\ \hline
    Rectangular                & BSV           & 1.992                     \\ \hline
                               & SVB           & 1.989                     \\ \hline
    \end{tabular}
    \caption{Empirical convergence rates obtained when decreasing $\mu$.}
    \label{table:empirical-convergence-reflections}
\end{table}

\begin{figure}
    \centering
    \includegraphics[ height=1.0\textheight]{figures/gaussianwave/BTSV-d1.pdf}
    \caption{BTSV $\sigma=2/\sqrt{3}$, $h=1$}
    \label{fig:btsv-Gaussian-h1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[ height=1.0\textheight]{figures/gaussianwave/BTSV-d4.pdf}
    \caption{BTSV $\sigma=2/\sqrt{3}$, $h=4$}
    \label{fig:btsv-Gaussian-h4}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[ height=1.0\textheight]{figures/gaussianwave/SVBT-d1.pdf}
    \caption{SVBT $\sigma=2/\sqrt{3}$, $h=1$}
    \label{fig:svbt-Gaussian-h1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[ height=1.0\textheight]{figures/gaussianwave/SVBT-d4.pdf}
    \caption{SVBT $\sigma=2/\sqrt{3}$, $h=4$}
    \label{fig:svbt-Gaussian-h4}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[ width=1.0\textwidth]{figures/gaussianwave/spectrum_vs_filter_bsv.pdf}
    \caption{Spectrum vs reflection coefficient BSV}
    \label{fig:spectrum_vs_filter_bsv}    
\end{figure}

\begin{figure}
    \centering
    \includegraphics[ width=1.0\textwidth]{figures/gaussianwave/spectrum_vs_filter_svb.pdf}
    \caption{Spectrum vs reflection coefficient BSV}
    \label{fig:spectrum_vs_filter_svb}    
\end{figure}




\begin{figure}
    \centering
    \includegraphics[ height=1.0\textheight]{figures/squarewave/SVBT-d1.pdf}
    \caption{SVBT $L=2/\sqrt{3}$, $h=1$}
    \label{fig:SVBT-rect-h1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[ height=1.0\textheight]{figures/squarewave/SVBT-d4.pdf}
    \caption{SVBT $L=2/\sqrt{3}$, $h=4$}
    \label{fig:SVBT-rect-h4}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[ width=1.0\textwidth]{figures/squarewave/spectrum_vs_filter_bsv.pdf}
    \caption{Spectrum vs reflection coefficient BSV}
    \label{fig:spectrum_vs_filter_bsv_rect}    
\end{figure}

\begin{figure}
    \centering
    \includegraphics[ width=1.0\textwidth]{figures/squarewave/spectrum_vs_filter_svb.pdf}
    \caption{Spectrum vs reflection coefficient SVB}
    \label{fig:spectrum_vs_filter_svb_rect}    
\end{figure}









































